MODS -- A USV-oriented object detection and obstacle segmentation benchmark

Small-sized unmanned surface vehicles (USV) are coastal water devices with a broad range of applications such as environmental control and surveillance. A crucial capability for autonomous operation is obstacle detection for timely reaction and collision avoidance, which has been recently explored in the context of camera-based visual scene interpretation. Owing to curated datasets, substantial advances in scene interpretation have been made in a related field of unmanned ground vehicles. However, the current maritime datasets do not adequately capture the complexity of real-world USV scenes and the evaluation protocols are not standardised, which makes cross-paper comparison of different methods difficult and hinders the progress. To address these issues, we introduce a new obstacle detection benchmark MODS, which considers two major perception tasks: maritime object detection and the more general maritime obstacle segmentation. We present a new diverse maritime evaluation dataset containing approximately 81k stereo images synchronized with an on-board IMU, with over 60k objects annotated. We propose a new obstacle segmentation performance evaluation protocol that reflects the detection accuracy in a way meaningful for practical USV navigation. Nineteen recent state-of-the-art object detection and obstacle segmentation methods are evaluated using the proposed protocol, creating a benchmark to facilitate development of the field. The proposed dataset, as well as evaluation routines, are made publicly available at vicos.si/resources.

==> tables/modb_obstacle_detection_results.tex <==
\begin{tabular}{ccccc}
 & Mask R-CNN & FCOS & YOLOv4 & SSD \\ \hline
\textit{Setup\textsubscript{1}} & \textbf{0.125} & 0.07 & 0.08 & 0.065 \\
\textit{Setup\textsubscript{2}} & \textbf{0.178} & 0.138 & 0.113 & 0.094 \\
\textit{Setup\textsubscript{3}} & 0.953 & \textbf{0.969} & 0.958 & 0.933
\end{tabular}

==> tables/modb_obstacle_detection_results_large.tex <==
% large
\begin{tabular}{c|c|c|c|c}
 & Mask R-CNN & FCOS & YOLOv4 & SSD \\ \hline
\textit{Setup\textsubscript{1}} & 0.260 & 0.163 & 0.269 & 0.249 \\ \hline
\textit{Setup\textsubscript{2}} & 0.522 & 0.483 & 0.431 & 0.43 \\ \hline
\textit{Setup\textsubscript{3}} & 0.96 & 0.965 & 0.955 & 0.939
\end{tabular}

==> tables/modb_obstacle_detection_results_medium.tex <==
% medium
\begin{tabular}{c|c|c|c|c}
 & Mask R-CNN & FCOS & YOLOv4 & SSD \\ \hline
$Setup_1$ & 0.209 & 0.117 & 0.183 & 0.142 \\ \hline
$Setup_2$ & 0.384 & 0.287 & 0.303 & 0.238 \\ \hline
$Setup_3$ & 0.953 & 0.976 & 0.972 & 0.941
\end{tabular}

==> tables/modb_obstacle_detection_results_small.tex <==
% small
\begin{tabular}{c|c|c|c|c}
 & Mask R-CNN & FCOS & YOLOv4 & SSD \\ \hline
$Setup_1$ & 0.068 & 0.034 & 0.024 & 0.022 \\ \hline
$Setup_2$ & 0.092 & 0.072 & 0.035 & 0.031 \\ \hline
$Setup_3$ & 0.962 & 0.969 & 0.927 & 0.915
\end{tabular}

==> tables/trainable_parameters_det.tex <==
% MODD2 DATASET

\small{
\resizebox{\ifdim\width>\columnwidth\columnwidth\else\width\fi}{!}{%
\begin{tabular}{lrr}
Architecture                                    & N$_\mathrm{param}$ & $\Delta_{t}$ [ms]\\
\midrule
SSD~\citep{liu2016ssd}                           & 24M           & 19.7 \\
Fcos~\citep{tian2019fcos}                        & 50M           & 69.3 \\
Yolo4~\citep{bochkovskiy2020yolov4}              & 61M           & 40.6 \\
MaskRCNN~\citep{he2017mask}                     & 63M           & 109.7 \\
\end{tabular}
}%
}
